Real-Time Event Detection with Random Forests and Temporal Convolutional Networks for More Sustainable Petroleum Industry

The petroleum industry is crucial for modern society, but the production process is complex and risky. During the production, accidents or failures, resulting from undesired production events, can cause severe environmental and economic damage. Previous studies have investigated machine learning (ML) methods for undesired event detection. However, the prediction of event probability in real-time was insufficiently addressed, which is essential since it is important to undertake early intervention when an event is expected to happen. This paper proposes two ML approaches, random forests and temporal convolutional networks, to detect undesired events in real-time. Results show that our approaches can effectively classify event types and predict the probability of their appearance, addressing the challenges uncovered in previous studies and providing a more effective solution for failure event management during the production.

==> 2-relwork_discard_.tex <==
\section{Related Work}
\label{sec:relwork}

\baifan{should be shortened, extra text move to the journal paper}

\noindent 
\textbf{Rate prediction.}https://www.overleaf.com/project/641c5f075c2eb1b782806dec#

~\cite{izgec2009real}When used in tandem with the Hall integral, the derivative curve, obtained either analytically or numerically, provides unambiguous diagnosis of a well's performance status. 

~\cite{yu2017method}It consists of three parts. The first step is deriving equation to calculate reasonable injection production rates by material balance equation. The second step is deducing formula to forecast water cut and oil production rate by relative empirical equation with production data. The last step is constructing an equation to calculate reasonable water injection rate with the above derived Eqs.

~\cite{deli2020data}Based on the traditional numerical simulation and optimization algorithms, in combination with the layered injection and production 'hard data' monitored at real time by automatic control technology, a systematic approach for detailed water injection design using data-driven algorithms is proposed. % ML as well
~\cite{}
~\cite{}

\medskip
\noindent
\textbf{ML in oil gas production.}

~\cite{aldhaheri2017development}:polymer gels have been proven to be effective in addressing water production problem and in increasing oil recoveries in mature oilfields. we utilized a machine-learning technique to develop an advanced selection methodology for the application of polymer gels in injection wells. \textbf{logistic regression technique}


~\cite{nwachukwu2018fast} Fast evaluation of well placements in heterogeneous reservoir models using machine learning. Accurate prediction of reservoir behavior in response to changes in control parameters is an important aspect of reservoir management and optimization. Full-physics numerical simulations currently provide the most accurate approach for estimating reservoir response and performance.. the use of the gradient boosting method for surrogate reservoir modeling.\textbf{Extreme Gradient Boosting}

~\cite{pratama2022well}With the increasing of water injection activities especially for marginal or stranded fields, the well pair analysis in routine water injection surveillance is crucial to understand the reservoir performance and identify opportunities to improve the ultimate oil recovery. This article aims to propose an alternative technique to evaluate the communication strength between injector-producer well pairs based on statistical and machine learning algorithms. The proposed technique is applied to an offshore water injection field located in the North Sea from open-source data. \textbf{Volve dataset. Random forest and support vector machine}


~\cite{liu2021application} \textbf{XGBoost } Interlayer water injection profile is an important data for oilfield development and adjustment. At present, it is mainly based on field test, with high cost and few data. XGBoost ensemble learning algorithm is used to realize small sample database prediction of longitudinal water injection profile in F oilfield.


~\cite{yan2022robust} \textbf{DL} predict multiphase flow behavior during geological CO2 injection.

~\cite{zhong2020predicting} \textbf{CNN, similar topic, have a look introduction} Waterflooding, during which water is injected in the reservoir to increase pressure and therefore boost oil production, is extensively used as a secondary oil recovery technology. Tracking the extent and efficacy of waterflooding (i.e., fluid distributions) is a primary task of reservoir engineers and is traditionally achieved by running full reservoir models. In this work, we design and implement a proxy model using a conditional deep convolutional generative neural network (cDC-GAN), which can be used to quickly calculate the dynamic fluid distribution of a heterogeneous reservoir under waterflooding. Zero-sum game theory is the basis for the cDC-GAN, which includes a pair of generative discriminative models.

~\cite{ma2019waterflooding} Recently, substantial technical progress has been made to solve complex tasks in the field of artificial intelligence (AI) by incorporating deep neural networks into reinforcement learning (RL). In this paper, four state-of-the-art deep RL algorithms are applied to optimize the net present value (NPV) of waterflooding (WF) under geological uncertainties by adjusting the water injection rate.

\textbf{Extremly relevant, water injection with different ML models (Artificial neural network, support vector machine, decision tree, random forest, and committee machine intelligent system)}~\cite{shafiei2022artificial}
